Knowledge Graph-based Session Recommendation with Adaptive Propagation

Session-based recommender systems (SBRSs) predict users' next interacted items based on their historical activities. While most SBRSs capture purchasing intentions locally within each session, capturing items' global information across different sessions is crucial in characterizing their general properties. Previous works capture this cross-session information by constructing graphs and incorporating neighbor information. However, this incorporation cannot vary adaptively according to the unique intention of each session, and the constructed graphs consist of only one type of user-item interaction. To address these limitations, we propose knowledge graph-based session recommendation with session-adaptive propagation. Specifically, we build a knowledge graph by connecting items with multi-typed edges to characterize various user-item interactions. Then, we adaptively aggregate items' neighbor information considering user intention within the learned session. Experimental results demonstrate that equipping our constructed knowledge graph and session-adaptive propagation enhances session recommendation backbones by 10%-20%. Moreover, we provide an industrial case study showing our proposed framework achieves 2% performance boost over an existing well-deployed model at The Home Depot e-platform.

==> concerns.tex <==
\section{Fairness Concerns in Online Dating Recommendations} 
\label{sec-concerns}
In Sec.~\ref{sec-analysis}, we analyzed complex user behaviors in a real-world online dating site with an emphasis on the users' opposite gender ratio, which provides a more fine-grained insight into their sexual orientations according to their historical interactions. 
%From Sec.~\ref{sec-analysis}, we have observed different types of users (i.e., of different genders and preferences) and interaction relationships. 
% \yw{Although it is good to connect with node-level or edge-level, we haven't defined anything related to node and edge before}
In this section, we seek to study whether these users (grouped by their sexual orientation) would be treated fairly if a recommender system were to be applied in an attempt to improve their user experience. Specifically, we first formally define the group unfairness based on the average performance gap between groups, then we perform an initial empirical evaluation on off-the-shelf recommendation algorithms to simulate whether unfairness was to exist in such a recommender system if deployed in the real world. %\td{note: can probably be shorter at the end}

%The natural question then arises whether these users are treated fairly if a recommender system is applied to improve users' experience. \td{here we do not necessarily want this to be that a natural question comes up from exploratory analysis, but that specifically we wanted to focus on this direction}
% by recommending partners a user might be interested in. 
% In this section, we begin our exploration by first quantifying the group unfairness based on groups split by sexual orientation and evaluating the existing recommender algorithms to investigate whether unfairness exists.
% first quantifying users' sexual orientation based on their historical interactions and then proposing the unfairness quantification. With the proposed measurements, we evaluate the existing recommender systems.
% \yw{I think here the novel-level and edge-level fairness is unclear to me, could we point this out in the related work - fairness in online dating?}
% \yy{change to user-level and interaction-level}


% \subsection{Users'  Sexual Orientations}
% % \yy{Note: need to find the right word for opposite gender. Not sure whether this is offensive.}

% Diversity exists in individuals' sexual orientation which describes a person's identity in relation to the gender/genders to which they are sexually attracted, leading to different groups of people including heterosexual, homosexual, bisexual, and etc. Although this identity might be filled in by the users for providing better recommendation quality in some online dating platforms, these categories are protected and are hard to obtain. Additionally, some users might be reluctant to share such information due to privacy concerns. However, the difference among the users will be revealed during the dating interactions where heterosexual users prefer to date more with the opposite gender while homosexual users prefer to date more with the same gender. It indicates that users with different sexual orientations have varying preferences toward the opposite gender. Based on this assumption, we use \textit{Opposite Gender Ratio (OGR)} as the indicator/pseudo label of users' sexual orientations. 
% \yy{have already mentioned sexual orientation here, merge the description of sexual orientation above}


% \subsection{User-Level Unfairness}
%\vspace{-0.5ex}
\subsection{User-based Group Unfairness}
% \yw{Following the existing literature that fairness can be interpreted as the equality of utility across entities in different groups, we define the node-level fairness in online dating recommendation as the difference of recommendation performance across users of different dating tastes, i.e., OGR. Intuitively, a larger gap in recommendation quality between users with varying levels of OGR indicates a higher discrimination/lower fairness of the recommender system in online dating. To quantify node-level unfairness, we divide users into multiple groups based on their OGR..... }
% \yw{I am not sure but would it be better to also define the edge-level unfairness since it is very similar following the definition of NUF and also broad the research scope to not only limited to node-level unfairness. But it would also be weird if we only define but not do anything with it}
% \yy{will change to user level and interaction level}

Following the existing literature that fairness can be interpreted as the equality of utility across entities in different groups (e.g., divided by gender or race)~\cite{fu2020fairness,li2021user,ekstrand2018all}, we define the user-based group unfairness in online dating recommendation as the difference of recommendation performance across users of various sexual orientations, i.e., OGR. Intuitively, a larger gap in the recommendation quality between users with varied levels of OGR indicates a higher discrimination/lower fairness of the recommender system in online dating. To quantify such unfairness, we divide users into multiple groups based on their OGR
% For users with different $\text{OGR}$, the recommendation quality should stay similar. This assumption is commonly used in existing literature where fairness has been interpreted as some form of equality across groups (e.g., gender, race) which is measured by utility performance~\cite{fu2020fairness,li2021user,ekstrand2018all}. In our case, the groups are divided based on users' sexual orientation, and the utility difference is computed based on recommendation metrics. Despite users' differences in their dating tastes, a recommender system should provide equally high-quality services. This leads to the problem of user-level unfairness when groups of users with varying levels of $\text{OGR}$ are treated discriminatorily regarding the recommendation quality. To quantify group unfairness, we divide users into groups based on $\text{OGR}$ 
(i.e., users in each group are within the same interval of $\text{OGR}$ where the interval range for each group is the same. e.g., a $3$-group partition would have users with $\text{OGR}$ in ranges $[0, \frac{1}{3}), [\frac{1}{3}, \frac{2}{3})$, and $[\frac{2}{3}, 1]$, respectively.) and measure the average performance gap among groups. Formally, it is defined as follows.
\vspace{-1.0ex}
\begin{definition}
\textbf{User-based Group Unfairness} measures the discrepancy of recommendation performance among different groups $\mathcal{G}$, which is defined as follows based on the average performance gap of certain metrics specified by $\text{X}$ (e.g., recall, F1, etc) among group pairs (other aggregation methods such as max can also be used):
% \begin{equation}
%     \Delta_{\text{X}}(\mathcal{G}) = \frac{\sum_{(G_1, G_2)\in \mathcal{G} \times \mathcal{G}}|Q_X(G_1)-Q_X(G_2)|}{(|\mathcal{G}||\mathcal{G}|-1)/2\cdot Q_X^{ave}},
% \end{equation}
\begin{equation}
    \Delta_{\text{X}}(\mathcal{G}) = \frac{\mathbb{E}_{(G_1, G_2)\in \mathcal{G} \times \mathcal{G}}|Q_X(G_1)-Q_X(G_2)|}{Q_X^{ave}},
    \label{eq.unfairness}
\end{equation}
where $(G_1, G_2)$ is a unique group pair (i.e., $G_1 \neq G_2$), and $Q_X(G_i)=\frac{\sum_{u \in G_i}q_x(u)}{|G_i|}$ is the average recommendation performance measured by metric $\text{X}$ of users in the group $G_i$ with $q_x(u)$ being user $u$'s performance according to metric X. The denominator normalizes by the average performance to mitigate the impact of performance scale across metrics where $Q^{\text{ave}}_X = \frac{\sum_{G \in \mathcal{G}}Q_X(G)}{|\mathcal{G}|}$.
% To mitigate the impact of the performance scale, we further update the above equation by dividing the average performance (i.e., $Q^{\text{ave}}_X = \frac{\sum_{G \in \mathcal{G}}Q_X(G)}{|\mathcal{G}|}$) of these groups.
% \yw{where do we use Q_{\text{ave}}?}
% \begin{equation}
%     Q_{\text{ave}} = \frac{\sum_{G \in \mathcal{G}}Q
%     (G)}{|\mathcal{G}|}
% \end{equation}


\end{definition}

Besides the \textit{user-based group unfairness}, due to the diversity of sexual orientations which leads to various types of interactions (e.g., $\overrightarrow{\text{FF}}$ and $\overrightarrow{\text{FM}}$), there are also concerns about \textit{interaction-based group unfairness} that different types of interactions should be treated similarity, which can be defined 
similarly to user-based, but left as one future work.
%in a similar way with the user-based one. 
% \td{adding italics here to emphasize the interaction-based?}
% \yy{sure, thanks}


% \subsection{Edge-Level Unfairness}

% Due to the diversity of sexual orientations, various types of dating interactions exist. Besides the most common interactions between Female-Male (F-M) and Male-Female (M-F), there are also homosexual interactions of Male-Male (M-M) and Female-Female (F-F). Similarly with Node-Level Unfairness, different types of edges should have similar quality of recommendation, raising up the concern of Edge-Level Unfairness.

% \begin{definition}
% \textbf{Edge-Level Unfairness ($\Delta_{\text{EUF}}$)} measures the discrepancy among different types of edges (i.e., F-M, M-F, M-M, F-F).

% \begin{equation}
%     \Delta_{\text{EUF}}=(\mathcal{G}^E) = \frac{\sum_{(G_1, G_2)\in \mathcal{G}^E \times \mathcal{G}^E}|Q^E(G_1)-Q^E(G_2)|}{(|\mathcal{G}||\mathcal{G}|-1)/2},
% \end{equation}
% where $\mathcal{G}^E$ denote all interactions from four types (i.e., M-M, F-F, M-F, and F-M), $Q^E(G_i)=\frac{\sum_{u \in G_i}q^E(u)}{|G_i|}$ is the average recommendation quality (e.g., ROC, AP) of edges in the group $G_i$ with $q^E(e)$ being the detailed recommendation quality metric of edge $e$. Similarly, we divide the equation by the average performance to mitigate the effect of scale among various metrics.

% \end{definition}



\subsection{Initial Fairness Evaluation in Online Dating Recommendation}
% \td{Preliminary Fairness Evaluation in Dating Recommendation} 
% \td{may consider changing this subsection }
In this section, we conduct an initial fairness evaluation to investigate whether user-based group unfairness exists in three representative recommender algorithms. We first introduce the dataset pre-processing steps, evaluation metrics, and the evaluated models. We then report the experimental results on the pre-processed dataset which reveal the consistent presence of group unfairness across algorithms. In the end, we discuss two potential na\"ive ``fixes" and the reason why they could not work, which urges the need to design a fair model. 
% \td{perhaps naive instead of easy ``fixes''}
% aim to answer whether user-level unfairness exists in recommender systems. 
% To answer this question, 
\subsubsection{Pre-processing}
To improve the data quality, we perform the following pre-processing steps: (1) Remove users without gender information as $\text{OGR}$ needs to be computed with the context of gender; (2) Filter edges whose rating is less than $10$ so that
% (i.e., only keep the highest rating) 
% which means that 
the remaining edges show strong preferences; (3) Apply k-core setting iteratively to remove users with interaction number smaller than $k=5$. After these steps, every user has at least five interactions, and then we randomly split the dataset into train/validation/test based on $60\%/20\%/20\%$ proportions so that at least one interacted user will be assigned to the validation and test dataset. To further ensure that different genders have the chance to be assigned to train/validation/test, we randomly split for genders (i.e., female and male) separately.

\vspace{-1ex}
\subsubsection{Evaluation Metrics} 
We include a wide range of common utility metrics~\cite{isinkaye2015recommendation} and their corresponding fairness metrics for a comprehensive comparison. The metrics include Recall@20 (R@20), Precision@20 (P@20), F1@20, Hit Ratio (H@20), and Normalized Discounted Cumulative Gain (NDCG, N@20). Their corresponding fairness metrics are computed according to Eq.~\ref{eq.unfairness}, which are denoted as $\Delta_\text{R}@20$, $\Delta_\text{P}@20$, $\Delta_\text{F1}@20$, $\Delta_\text{H}@20$, and $\Delta_\text{N}@20$, respectively. Note that for utility (fairness) metrics, the higher (lower) the value, the better the performance.
% \yy{todo: unify the notations with the above section}

\vspace{-1ex}
\subsubsection{Evaluated Models}
We evaluate the fairness and utility performances across three representative recommender models,
% \yw{recommendation models:, I think the next sentence could be removed}, 
which include seminal works and current state-of-the-art: %\td{(essentially the comment after the methods on user-item to user-user we might consider earlier and then just present them in a user-user/generalized way...)...need to think about this here if we want to first discuss the relation of giving/receiving ratings in online dating provides two user perspectives to the same node as compared to in other settings such as e-commerce }: 

% \td{note:...} %\td{for now do not say where the code is from, instead, just later include a link to your anonymous code that includes the code from the cagcn repo but perhaps a comment inside the files from there, e.g., ``Note that this file has been modified from the file https://github.com/yuwvandy/cagcn/...'' it looks better to just have the anonymous repo at this point since directly linking to just one repo for cagcn that was just released/accepted would provide them insights to who the authors might be}\yy{sure, this makes sense.}
% We evaluated the performance of three baseline models, which are widely adopted for recommendation where the implementation is based on this repository\footnote{\url{https://github.com/yuwvandy/cagcn}}:
% \yw{All below definitions are based on user-item, how do you modify it to also work on user-user data? I think we need to specify this.}\yy{updated along with the bpr loss}
% \yy{here I adjusted the model description with Yi's writing in related work. Thank you @Yi.}
\vspace{-1.5ex}
\begin{itemize}[leftmargin=5ex]
    \item \textbf{Matrix Factorization (MF)}~\cite{rendle2012bpr} 
    is a simple yet effective method to predict interaction scores between entities and consequently top-k recommendations. The objective is generally to find entity embeddings whose dot product best resembles their sparsely observed interactions.
    %is a simple yet effective method to predict the user-item interaction score and consequently recommend items to users. The objective is to find the user and item embedding whose dot product best resembles the sparsely observed interactions.
% In matrix factorization, the objective is to find the user embedding $v_{u}$, and the item embedding $v_i$ that after multiplication, can best resemble the sparse observed ratings $r_{u i}$.
    % \item \textbf{Matrix Factorization (MF)}~\cite{rendle2012bpr}: This is one of the most classical models leveraging collaborative filtering (CF) to learn the user and item representations. It utilizes a Bayesian Personalized Ranking (BPR) loss to preserve the user's ranking over the interacted items.
    \item \textbf{Neural Graph Collaborative Filtering (NGCF)}~\cite{wang2019neural} is the first GNN-based model to leverage the collaborative filtering (CF) effect for recommendations, which utilizes higher-order connectivities of history interactions. Entities aggregate the neighborhood information with the message-passing mechanism. The learned embeddings from various layers are concatenated and used to predict entity interactions.
    % This is the first GNN-based model to leverage the collaborative filtering effect for recommendations, which utilizes higher-order connectivities of user-item interactions. User and item aggregate the neighborhood information with the message-passing mechanism. The learned embeddings from various layers are concatenated and used to predict the user-item interaction. 
    % \item \textbf{LightGCN}~\cite{he2020lightgcn}: This model advances NGCF by simplifying the feature propagation process. It removes the linear transformation and nonlinear activation steps. It is one of the most popular GNN-based collaborative filtering models.
    % \item \textbf{CAGCN}~\cite{wang2022cagcn}:
    \item \textbf{$\text{Collaboration-Aware Graph Convolutional Network (CAGCN}^*\text{)}$}~\cite{wang2022cagcn} is a fusion model of LightGCN~\cite{he2020lightgcn} and CAGCN~\cite{wang2022cagcn} which inherits the benefits from these two models and has better performance. LightGCN advances NGCF by simplifying the feature propagation process, which removes the linear transformation and nonlinear activation steps. CAGCN analyzes how message-passing captures CF effect and proposes a recommendation-oriented topological metric, Common Interacted Ratio (CIR), for collaboration-aware propagation.
    % This model is a fusion model of LightGCN~\cite{he2020lightgcn} and CAGCN~\cite{wang2022cagcn} which shows a better performance than both of them. LightGCN advances NGCF by simplifying the feature propagation process, which removes the linear transformation and nonlinear activation steps. CAGCN analyzes how message-passing captures the collaborative effect and proposes a recommendation-oriented topological metric, Common Interacted Ratio (CIR), which is used in the propagation. $\text{CAGCN}^*$ inherits the benefits from both these two models.
\end{itemize}

Although these algorithms are commonly used in settings with both user and item entities (i.e., user-item interactions), they are easily adapted to user-user interactions (e.g., friend/dating recommendations).
%These algorithms are commonly used for predicting user-item interactions which can be easily extended to user-user interaction in the dating recommendation. 
Specifically, they can be optimized with Bayesian Personalized Ranking (BPR) loss~\cite{rendle2012bpr} as follows:
\vspace{-0.25ex}
\begin{equation}
    \mathcal{L}_{\text{BPR}} = -\sum_{(u, i, j) \in \mathcal{D}}\log\sigma(\hat{y}_{ui}-\hat{y}_{uj})+\lambda_{\Theta}\|\Theta\|^2,\label{eq.bpr}
\end{equation}
% \td{where $\mathcal{D}$ denotes the training data of tuples $(u, i, j)$}
where $\mathcal{D}=\{(u,i,j)|u\in\mathcal{U}\land i\in I_u^+\land j\in I_u^-\}$ is the training dataset where $\mathcal{U}$ is the total user set who will receive the recommendation, $I_u^+$ is the user set that user $u$ has interacted with, and $I_u^-$ is the user set that user $u$ has not interacted with.
% Tuple $(u, i, j)$ denotes the center user $u$ who will receive the recommendation, the user $i$ who has been interacted with by user $u$, and the user $j$ who has not been interacted with
$\sigma(\cdot)$ is sigmoid function, and $\Theta$ denoted the model parameter with $\lambda_{\Theta}$ controlling the $L_2$ norm of ${\Theta}$ to prevent over-fitting.
% $\|\Theta\|^2$ is a $L_2$ regularization term to prevent overfitting. 
$\hat{y}_{ui}$ is the predicted preference/relevance score of user $u$ over the other user $i$ calculated by $\hat{y}_{ui}=\mathbf{h}_u \cdot \mathbf{g}_i$ where $\mathbf{h}_u$ represents the user $u$'s role in actively rating others, and $\mathbf{g}_i$ represents the user $i$'s property of being rated. 
% {positive (real) interaction from user $u$ to user $i$ and a negative (imaginary) interaction to user $j$ denotes the center user who will receive the recommendation, the user who has been interacted with by user $u$, and the user who has not been interacted with, $\sigma(\cdot)$ is a sigmoid function, } 
% \td{perhaps you can rewrite this part...notnecessary to go into too much detail, but just D defined and making sure the tuple description specifically highlights the role of i and j (your previous was just according to the order but can add the notation specifically in teh text when describing them}
% where tuple $(u, i, j)$ denotes the center user who will receive the recommendation, the user who has been interacted with by user $u$, and the user who has not been interacted with, $\sigma(\cdot)$ is a sigmoid function, and $\|\Theta\|^2$ is a $L_2$ regularization term \td{(controlled by $\lambda_\theta$) ... can add this to the above} to prevent overfitting. $\hat{y}_{ui}$ is the predicted preference/relevance score of user $u$ over the other user $i$ calculated by $\hat{y}_{ui}=\mathbf{h}_u \cdot \mathbf{g}_i$ where $\mathbf{h}_u$ represents the user $u$'s role in actively rating others, and $\mathbf{g}_i$ represents the user $i$'s property of being rated. 
Minimizing this loss enhances the similarity between the center user and their interacted users and reduces the similarity with their un-interacted users. In this way, the learned embeddings well-represent the user's roles of rating others and being rated, such that the dot product indicates the user's preference towards other users. 



\subsubsection{Evaluation Results}
To mitigate the randomness impact for a better comparison, we run the evaluated models $5$ times with different seeds and report the average results where without specification, the group number is set to $3$. The model selection is based on the average utility score, $\text{Avg Utility}=\frac{\text{R}@20+\text{P}@20+\text{F1}@20+\text{H}@20+\text{N}@20}{5}$, on validation data.
% \yw{on validation data. Also note the font here is not aligned with previous one.}

The average utility result for three groups divided by OGR is shown in Fig.~\ref{fig:baselines} with the detailed statistical overall result shown in Appendix~\ref{sec.baseline-and-fair-model-selection}. 
% In Fig.~\ref{fig:baselines}, we plot the average utility performance for three groups divided by OGR. The ranges of OGR for groups $G_1/G_2/G_3$ are $[0, \frac{1}{3}), [\frac{1}{3}, \frac{2}{3}), [\frac{2}{3}, 1]$ respectively. 
From the figure, we observe that generally, $G_3$ has better performance than 
% \yz{use "than do"} 
$G_1$ and $G_2$, indicating that $G_3$ enjoys better recommendation quality compared with the other groups. The performance gap among groups is quantified by the proposed unfairness measurement where these models have more than $0.5$ unfairness scores (i.e., $0.5449$ for MF, $0.5692$ for NGCF, and $0.5635$ for CAGCN$^*$. The detailed results are shown in Appendix~\ref{sec.baseline-and-fair-model-selection}), presenting a consistent unfairness that appears to be algorithm/model-agnostic according to our results.
%for groups across algorithms.

\begin{figure}[htbp]
    \centering
    \vskip -0.23cm
    \includegraphics[width=0.97\textwidth]{Figures/baseline_performance.png}
    \vskip -0.4cm
    \caption{Utility performance across three models on five metrics per group, which are divided based on even width bins for discretizing OGR into three groups ($G_1=\{u|\text{OGR}_u\in [0, \frac{1}{3})\}$
    % $\{\text{OGR}_u\in [0, \frac{1}{3})|u\in G_1\}$ 
    with $G2$, $G3$ similarly defined). 
    % $G_1$/$G_2$/$G_3$ are more towards homosexual/bisexual/heterosexual, respectively. 
    $G_3$ consistently has better performance.}
    
    %PREVIOUS --> \caption{Group performance of five utility metrics across three baselines where groups are divided based on even width bins for discretizing OGR into three groups ($G_1=\{u|\text{OGR}_u\in [0, \frac{1}{3})\}$
    % % $\{\text{OGR}_u\in [0, \frac{1}{3})|u\in G_1\}$ 
    % with $G2$ and $G3$ similarly defined). 
    % % $G_1$/$G_2$/$G_3$ are more towards homosexual/bisexual/heterosexual, respectively. 
    % $G_3$ consistently has better performance in all the metrics.}
    % \yw{) or ] in interval specification?}
    
    \label{fig:baselines}
    \vskip -2.5ex
\end{figure}
% change the x-axis to groups (done)
% \td{only one legend for blue=mf, orange=ngcf, green=lightgcn is needed for these that can go across the top/bottom, could also consider adding in either the figure legend area what the G1, G2, G3 are defined to be (since it would not take up too much space and make it easier to quickly know the groups for both this figure and throughout the work if it were to be missed in the main text. we can consider also adding a takeaway one or two sentences in the figure caption to make it easier for the reader as compared to only in the main text} 
% \yy{Sure, will update it when having the updated result with more models. Do you mean legends like G1: homosexual-alike (i.e., OGR $\in [0, \frac{1}{3}])$, G2... }
% \yy{If the fair model selection did not improve a lot of the fairness, it then motivates us to design a fair model since only fair model selection is not effective.}
% \yy{To be included: (1) a table of average utility and fairness measurement; (2) a figure showing the u-shape with three bars related to three models}
% based on old split
% \begin{table}[htbp]
% \setlength{\extrarowheight}{.5pt}
% \setlength\tabcolsep{1.5pt}
% \caption{Performance Comparison (the $\uparrow$ represents the larger the better and $\downarrow$ represents the opposite).}
% \vskip -1.75ex
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \Xhline{1\arrayrulewidth}
% Metric & MF & NGCF & LightGCN & Fair MF & Fair NGCF & Fair LightGCN\\
% \Xhline{1\arrayrulewidth}
% R@20$\uparrow$ & $0.2748\pm0.0013$ & $0.2777\pm 0.0010$ & $0.3027\pm 0.0010$ & $0.2695\pm0.0047$ & $0.2771\pm0.0011$ & $0.2970\pm0.0050$ \\
% P@20$\uparrow$ & $0.1883\pm0.0002$ & $0.1887 \pm 0.0001$ & $0.2195 \pm 0.0001$ & $ 0.1843\pm0.0009 $ & $ 0.1869\pm0.0003 $ & $ 0.2135\pm0.0016 $ \\
% F1@20$\uparrow$ & $0.0503\pm0.0003$ & $0.0512 \pm0.0002$ & $0.0575 \pm0.0001 $ &$0.0494 \pm 0.0015$  & $ 0.0511\pm 0.0003$ & $ 0.0555\pm0.0021 $\\
% H@20$\uparrow$ &$0.5526\pm0.0021$ & $0.5597 \pm 0.0014$ & $ 0.5914\pm 0.0010$ & $ 0.5488\pm 0.0038$ &$ 0.5567\pm 0.0042$ &$ 0.5861\pm 0.0050$ \\
% N@20$\uparrow$ &$0.0728\pm0.0012$ & $0.0741 \pm 0.0016$ & $ 0.0824\pm 0.0006$ & $ 0.0713\pm 0.0022$ & $ 0.0739\pm 0.0022$ & $0.0797 \pm 0.0047$\\
% \Xhline{1\arrayrulewidth}
% Avg Utility$\uparrow$ &$0.2277\pm0.0009$ & $0.2303 \pm 0.0007 $ & $ 0.2507\pm 0.0005$ &$ 0.2247\pm 0.0026$  &$ 0.2291\pm 0.0016$ &$ 0.2464\pm0.0036 $\\
% \Xhline{1\arrayrulewidth}
% RF@20$\downarrow$ &$0.0873\pm0.0142$ & $ 0.1332\pm 0.0307 $ & $ 0.0599\pm 0.0067$ &$ 0.0920\pm 0.0172$ & $ 0.1227\pm  0.0294$&$ 0.0728\pm 0.0264$\\
% PF@20$\downarrow$ &$0.2483\pm0.0399$ & $ 0.3266\pm 0.0433 $ & $ 0.2226\pm 0.0283$ &$ 0.2631\pm 0.0424$ &$ 0.3195\pm 0.0359$ & $ 0.2199\pm 0.0495$\\
% F1F@20$\downarrow$ &$0.7671\pm0.0398$ & $ 0.8145\pm 0.0384$ & $ 0.7475\pm 0.0273$ &$ 0.7652\pm 0.0436$ &$ 0.8120\pm 0.0300$ & $ 0.7265\pm 0.0486$\\
% HF@20$\downarrow$ &$0.4329\pm0.0414$ & $ 0.4887\pm 0.0347$  &$ 0.3855\pm 0.0227$  &$ 0.4396\pm 0.0403$ &$ 0.4818\pm 0.0265$ & $ 0.3862\pm 0.0459$\\
% NF@20$\downarrow$ &$0.6323\pm0.0328$ & $ 0.6888\pm 0.0287$  &$ 0.6130\pm 0.0323$ &$ 0.6304\pm 0.0443$ &$ 0.6850\pm 0.0401$ & $ 0.5944 \pm0.0377 $\\
% \Xhline{1\arrayrulewidth}
% Avg Fairness$\downarrow$ & $0.4336\pm0.0276$& $ 0.4904\pm0.0346 $ &$ 0.4057\pm 0.0223$ &$ 0.4381\pm 0.0335$ &$ 0.4842\pm 0.0275$ & $ 0.4000\pm 0.0329$\\
% \Xhline{1\arrayrulewidth}
%  \end{tabular}
%  \vskip -2.5ex
% \label{tab-model-result}
% \end{table}
% new split
% MF:
% Utility: [0.2002 0.0499 0.069  0.5406 0.1517]
% Fairness: [0.4964 0.7361 0.6397 0.3861 0.4664]
% utility std: [0.0006 0.0002 0.0003 0.0007 0.0014]
% fairness std: [0.0107 0.0134 0.011  0.0137 0.0175]
% Utility: 0.2023 Fairness: 0.5449
% avg utility std: 0.0005 avg fairness std: 0.0121
% NGCF
% Utility as model selection
% (5, 11)
% (5,)
% Utility: [0.2019 0.0508 0.0701 0.5457 0.1527]
% Fairness: [0.5294 0.7577 0.6611 0.4016 0.4961]
% utility std: [0.0009 0.0002 0.0002 0.002  0.0012]
% fairness std: [0.0126 0.0207 0.0166 0.0118 0.0157]
% Utility: 0.2043 Fairness: 0.5692
% avg utility std: 0.0009 avg fairness std: 0.0135
% LightGCN
% Utility as model selection
% (5, 11)
% (5,)
% Utility: [0.2209 0.0567 0.0778 0.5774 0.1781]
% Fairness: [0.4818 0.7208 0.6243 0.3592 0.4587]
% utility std: [0.0004 0.0001 0.0001 0.0008 0.0003]
% fairness std: [0.0085 0.0208 0.0096 0.0111 0.0151]
% Utility: 0.2222 Fairness: 0.529
% avg utility std: 0.0002 avg fairness std: 0.0115
% \begin{table}[htbp]
% \setlength{\extrarowheight}{.5pt}
% \setlength\tabcolsep{1.5pt}
% \caption{Performance Comparison (the $\uparrow$ represents the larger the better and $\downarrow$ represents the opposite).}
% \vskip -1.75ex
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \Xhline{1\arrayrulewidth}
% Metric & MF & NGCF & LightGCN & Fair MF & Fair NGCF & Fair LightGCN\\
% \Xhline{1\arrayrulewidth}
% R@20$\uparrow$ & $0.2002\pm0.0006$ & $0.2019\pm0.0009 $ & $0.2209\pm 0.0004$ & $\pm$ & $\pm$ & $\pm$ \\
% P@20$\uparrow$ & $0.0499\pm0.0002$ & $0.0508\pm0.0002 $ & $0.0567\pm 0.0001$ & $\pm$ & $\pm$ & $\pm$ \\
% F1@20$\uparrow$ & $0.0690\pm0.0003$ & $0.0701\pm 0.0002$ & $0.0778\pm 0.0001$ & $\pm$ & $\pm$ & $\pm$ \\
% H@20$\uparrow$ & $0.5406\pm0.0007$ & $0.5457\pm 0.0020$ & $0.5774\pm 0.0008$ & $\pm$ & $\pm$ & $\pm$ \\
% N@20$\uparrow$ & $0.1517\pm0.0014$ & $0.1527\pm0.0012 $ & $0.1781\pm0.0003 $ & $\pm$ & $\pm$ & $\pm$ \\
% \Xhline{1\arrayrulewidth}
% Avg Utility$\uparrow$ & $0.2023\pm0.0005$ & $0.2043\pm0.0009 $ & $0.2222\pm 0.0002$ & $\pm$ & $\pm$ & $\pm$ \\
% \Xhline{1\arrayrulewidth}
% RF@20$\downarrow$ & $0.4964\pm0.0107$ & $0.5294\pm 0.0126$ & $0.4818\pm 0.0085$ & $\pm$ & $\pm$ & $\pm$ \\
% PF@20$\downarrow$ & $0.7361\pm0.0134$ & $0.7577\pm0.0207 $ & $0.7208\pm 0.0208$ & $\pm$ & $\pm$ & $\pm$ \\
% F1F@20$\downarrow$ & $0.6397\pm0.0110$ & $0.6611\pm0.0166 $ & $0.6243\pm 0.0096$ & $\pm$ & $\pm$ & $\pm$ \\
% HF@20$\downarrow$ & $0.3861\pm0.0137$ & $0.4016\pm0.0118 $ & $0.3592\pm 0.0111$ & $\pm$ & $\pm$ & $\pm$ \\
% NF@20$\downarrow$ & $0.4664\pm0.0175$ & $0.4961\pm0.0157 $ & $0.4587\pm 0.0151$ & $\pm$ & $\pm$ & $\pm$ \\
% \Xhline{1\arrayrulewidth}
% Avg Fairness$\downarrow$ & $0.5449\pm0.0121$ & $0.5692\pm0.0135 $ & $0.5290\pm 0.0115$ & $\pm$ & $\pm$ & $\pm$ \\
% \Xhline{1\arrayrulewidth}
%  \end{tabular}
%  \vskip -2.5ex
% \label{tab-model-result}
% \end{table}
% \yy{plan to change the table format so that we can make more use of the single-column space}
% \yy{no need to include the table here, since it is a preliminary result and the previous figure should be sufficient, the result table can be put into appendix->will merge it with table2 (the reweighting result)}
% updated
 % \td{as here we do not want to emphasize too much that we have ``Model'' and ``Fair Model'', since this is still preliminary evaluation and not the final models and performances, so maybe something like saying this is something like ``Performance comparison of traditional model selection versus fairness-aware model selection across various backbone models (the $\uparrow$ represents ...). so in this way we then have a row above MF, NGCF, LightGCN that says ``Traditional Model Selection'' and one above them on the right side with ``Fairness-aware Model Selection''... or having MF (and each other model) contain two performances of (X, Y) where X is traditional utility-driven and Y is fairness-aware (instead of separating them and then the traditional and fairness are right next to each other for easy comparison) also, if switching to this type of (X,Y) setup the +- can be removed and just adding a note that says it is omitted since they were on average Z (which may end up being something like +- 1\%)} \yy{This is a very good suggestion! Since it is not the core results, maybe we can remove the std even without the average. Because it seems to be not so important here.}
 
% We also investigate the fairness-aware variants by changing the model selection criterion, we use $\text{score} = \text{Avg Utility}-\text{Avg Fairness}$ where $\text{Avg Fairness}$ is obtained in a similar way with $\text{Avg Utility}$ by averaging the fairness metrics. The detailed results for MF/NDCG/$\text{CAGCN}^*$ and their variants based on the fairness-aware model selection are shown in Appendix~\ref{sec.baseline-and-fair-model-selection}. 
% From the results, we observe that (1) When comparing MF/NGCF/$\text{CAGCN}^*$, despite their differences in the utility performance, all models have an unfairness score larger than $0.5$; (2) When comparing the model selected according to utility performance and the fairness-aware criterion, the improvement in fairness is not significant and unstable (The fairness performance improves a little for MF and $\text{CAGCN}^*$ while decreasing for NGCF.) This means that unfairness among different groups exists in these models, and simply changing the model selection to consider fairness is insufficient to find a fair model. Additionally, for MF and $\text{CAGCN}^*$, we observe an improvement of fairness with a decrease in utility performance where different platforms might have different demands, which raises the concern of whether the fairness-aware model selection can offer a good trade-off between utility and fairness. This raises the requirements for designing a new fair model and a more flexible model selection strategy.



% \begin{table}[htbp]
% \setlength{\extrarowheight}{1pt}
% \setlength\tabcolsep{3pt}
% \caption{...might consider a thin table showing fairness results...}
% \footnotesize
% \vskip -2ex
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \Xhline{1\arrayrulewidth}
%  & $\Delta_{\text{R}}@20$ & $\Delta_{\text{P}}@20$ & $\Delta_{\text{F1}}@20$ & $\Delta_{\text{H}}@20$ & $\Delta_{\text{N}}@20$ & Avg Fairness \\

% \Xhline{1\arrayrulewidth}
% MF &    &   &   &   &   &  a \\ 

% \Xhline{1\arrayrulewidth}
% NGCF &    &   &   &   &   & b  \\ 

% \Xhline{1\arrayrulewidth}
% $\text{CAGCN}^*$ &    &   &   &   &   & c \\ 

% % Metric & MF & NGCF & $\text{CAGCN}^*$ \\

% % \Xhline{1\arrayrulewidth}
% % R@20$\uparrow$ & $(0.2002, 0.1982)$ & $(0.2019, 0.1999) $  & $(0.2267, 0.2228)$ \\

% % P@20$\uparrow$ & $(0.0499, 0.0495)$ & $(0.0508, 0.0503) $ & $(0.0580, 0.0554)$ \\

% % F1@20$\uparrow$ & $(0.0690, 0.0684)$ & $(0.0701, 0.0696)$  & $(0.0798, 0.0767)$ \\

% % H@20$\uparrow$ & $(0.5406, 0.5363)$ & $(0.5457, 0.5382)$  & $(0.5890, 0.5850)$ \\

% % N@20$\uparrow$ & $(0.1517, 0.1498)$ & $(0.1527, 0.1497)$  & $(0.1802,0.1766 )$ \\

% % \Xhline{1\arrayrulewidth}
% % Avg Utility$\uparrow$ & $(0.2023, 0.2004)$ & $(0.2043, 0.2015) $  & $(0.2267,0.2233 )$\\

% % \Xhline{1\arrayrulewidth}
% % RF@20$\downarrow$ & $(0.4964, 0.4909)$ & $(0.5294, 0.5398)$  & $(0.5196, 0.4800)$ \\

% % PF@20$\downarrow$ & $(0.7361, 0.7241)$ & $(0.7577, 0.7786) $  & $(0.7534, 0.6996)$  \\

% % F1F@20$\downarrow$ & $(0.6397, 0.6319)$ & $(0.6611, 0.6840) $  & $(0.6562, 0.6082)$ \\

% % HF@20$\downarrow$ & $(0.3861, 0.3831)$ & $(0.4016, 0.4218) $  & $(0.3929, 0.3591)$ \\

% % NF@20$\downarrow$ & $(0.4664, 0.4566)$ & $(0.4961, 0.5203)$ & $(0.4955, 0.4547)$ \\

% % \Xhline{1\arrayrulewidth}
% % Avg Fairness$\downarrow$ & $(0.5449, 0.5373)$ & $(0.5692, 0.5889)$ & $(0.5635, 0.5203)$ \\
%  \Xhline{1\arrayrulewidth}
%  \end{tabular}
%  \vskip -2.5ex
% \label{tab-model-fairness}
% \end{table}



    
%\subsubsection{Potential Na\"ive ``Fix''}
%\td{Potential Na\"ive ``Fix'' Towards Fairness?}
\subsubsection{Potential Na\"ive ``Fix'' Towards Fairness}
In addressing the unfairness issue, one potential approach could be %to design 
a fairness-aware model selection. For example, it might be a quick and easy fix to use $\text{score} = \text{Avg Utility}-\text{Avg Fairness}$, where $\text{Avg Fairness}$ is obtained by averaging the fairness metrics, to replace the original utility-based model selection (i.e., $\text{Avg Utility}$). We conduct such an experiment whose detailed results are shown in Appendix~\ref{sec.baseline-and-fair-model-selection} and find there is no significant fairness improvement compared with the baseline models with the utility-based criterion for model selection. This indicates that simply considering fairness in the model selection is insufficient to achieve a fair model. Another potential solution would be to train the recommender system separately for different groups. However, it presents two challenges. First, it will further exacerbate the data sparsity issue, and such an issue would be more severe for the minority than the majority. Secondly, in the real-world scenario, a user in one group might be interested in a user from another group. Training the recommendation system in a separate manner would result in the restricted ability of only recommending users within one group and lead to a suboptimal outcome.
% a user in one group is not necessary to only reach out to users within the same group in the real world.
% guaranteed to not reach out to the user in another group in the real world. 
% If we train the system separately, it means that we can only recommend the users within one group, which restricts the potential partners from other groups and leads to a suboptimal outcome.
Therefore, both potential na\"ive ``fixes" indeed cannot fix the problem, since they are insufficient to find a fair model. This raises the requirements for designing a new fair model, such as based on in-processing and/or their combination with pre-processing/post-processing, which we present in the next section.
% \td{so thinking here the model selection can be thought of as post-processing, and data splitting can be thought of as pre-processing... perhaps these terms can be injected in this part?} \td{not necessary, but might connect the dots better between the related work, the preliminary, and more advanced ways proposed}




==> model.tex <==
\vspace{-1.25ex}
\section{Fair Recommender System}
\label{sec-model}
In this section, we analyze the potential causes of unfairness %for the unfairness problem 
where the recommendation performance differs among groups. We posit that it is related to group data imbalance and calibration imbalance. To improve fairness and mitigate these issues, we introduce two strategies: Re-weighting and Re-ranking. They can be used individually or simultaneously. 
% \yz{If time permits, please change "User Number" to "Number of Users" as indicated in the Slack Channel.}
\begin{figure}[htbp]
    \centering
    \vskip -0.5ex
    \includegraphics[width=0.75\textwidth]{Figures/causes.png}
    \vskip -0.5cm
    \caption{Two potential causes of unfairness: (a) group data imbalance, $G_3$ is the majority group which takes up the largest proportion, and $G_1$ and $G_2$ are the minority groups; (b) calibration imbalance, $G_1$ and $G_2$ have poorer calibration than $G_3$.}
    \label{fig:unfairness_reasons}
    \vskip -2.5ex
\end{figure}
% \yy{note, will update the figure to include a and b}
% \yy{when updating the figure, remember to decrease the bar width in (a)}

\vspace{-1.25ex}
\subsection{Re-weighting Towards Fairness: Mitigating Group Data Imbalance}
The issue of class imbalance, where the number of training instances per class is imbalanced, has been widely investigated across various domains~\cite{johnson2019survey, chawla2002smote}.
% \cite{wang2022imbalanced, chawla2002smote} \td{cite an imbalance classification survey and not wang2022imbalance, that can be added after acceptance so as to not provide further insights to them on who the authors are of this work}. 
During the training process, to achieve an overall higher utility performance, the majority class is typically optimized more than the minority class, leading to a performance gap. As shown in Fig.~\ref{fig:unfairness_reasons}(a), in our setting, the numbers of users in different groups are imbalanced. As a consequence, there are performance gaps among majority and minority groups, resulting in unfairness.
% resulting in group data imbalance and thus the performance gap between the majority and minority groups.
% Class imbalance issue has been widely investigated in various domains where the instance number in each class is imbalanced~\cite{wang2022imbalanced, chawla2002smote},
% \yw{could cite some of our imbalance work and also some also works}, 
% and the majority will generally have better performance than the minority. 
% Take two classes as an example: one is the majority, and another one is the minority. 
% During the training, in order to achieve a higher overall performance, the majority will be optimized more, while the minority will be less trained, resulting in a gap between the performance of the majority and the minority. 
% We have a similar case here where the number of users in different groups is imbalanced (i.e., $G_3$ has much more users than $G_1$ and $G_2$ as shown in Fig.~\ref{fig:unfairness_reasons} (a)), leading to the data imbalance which further leads to the performance gap. 
To mitigate this unfairness, we employ the re-weighting strategy, which has been utilized to address the class imbalance issue. This approach adjusts the focus of training by updating the weights based on the number of users in each group effectively balancing the original loss function accordingly such that equitable emphasis is put on each group when updating the model's parameters.
% \td{such that equitable emphasis is put on each group when updating the model's parameters (note: changed here to equitable as it seems like below the weights are not set to make the weight emphasis during training exactly fair, which makes sense)}. 
%\td{such that equal emphasis is put on each group when updating the model's parameters}. 
% This helps reduce the performance gap between the majority and minority groups and mitigate the fairness concerns raised in Sec.~\ref{sec-concerns}.
% This motivates us to utilize the re-weighting strategy, which has been applied to solve the class imbalance issue, to adjust the focus during training to reduce the performance gap between the majority and minority and thus mitigate the fairness concern raised in Sec~\ref{sec-concerns}. More specifically, we adjust the original loss to consider the weight based on the user number in each group.

% \yy{Should the weight be based on the user number in each group or the user appearance in the tuples? Generally, I think they would have a similar performance. Users in G0 and G1 also have lower degrees. I will also do this experiment. Similar to node-based and edge-based.}

% The loss used in the baselines above is the Bayesian Personalized Ranking (BPR) loss~\cite{rendle2012bpr}, which is defined as follows:
% \begin{equation}
%     \mathcal{L}_{\text{BPR}} = -\sum_{(u, i, j) \in \mathcal{D}}\log\sigma(\hat{y}_{ui}-\hat{y}_{uj})+\lambda_{\Theta}\|\Theta\|^2,
% \end{equation}
% where tuple $(u, i, j)$ denotes the user, positive item, and negative item, $\hat{y}_{ui}$ is the predicted preference score of user $u$ over item $i$, $\sigma(\cdot)$ is a sigmoid function, and $\|\Theta\|^2$ is a $L_2$ regularization term to prevent overfitting. Minimizing this loss aims to increase the similarity between the user and the positive item representations and decrease the similarity between the user and the negative item representations. In this way, the learned embeddings can represent the user and item features, such that the dot product between them could indicate the user's preference towards that item. Therefore, we can use it to predict the items the user will like for recommendation.\yw{Could this paragraph be moved to the preliminary?}

According to $\mathcal{L}_{\text{BPR}}$ in Eq.~\ref{eq.bpr}, each tuple is trained equally without consideration of the sizes of the groups. %user number in the groups. 
Generally, as one group (e.g., majority user group) appears more in the training data during the optimization, the users belonging to this group will achieve better performance as they share common (group-level) user behaviors.
%Generally, users in $G_3$ will be trained more to achieve better performance. 
To remedy this, we add a weight term for adjustment. The updated loss is as follows:
\begin{equation}
    \mathcal{L}_{\text{BPR}}^{\text{re-weighting}} = -\sum_{(u, i, j) \in \mathcal{D}} w_{G(u)} \log\sigma(\hat{y}_{ui}-\hat{y}_{uj})+\lambda_{\Theta}\|\Theta\|^2,
\end{equation}
where $w_{G(u)}$ is the weight for user $u$ based on $u$'s group, and the other notations share the same meaning as in Eq.~\ref{eq.bpr}.
% group this user belongs to. 
Generally, when $u$ belongs to a group with a larger user number (e.g., $G_3$), the weight will be lower than the case when $u$ belongs to one with a smaller user number (e.g., $G_1$ and $G_2$) to promote the training for minority user groups.
%minorities.
There have been well-established and commonly-used designs in practice for computing the weights~\cite{johnson2019survey},
% \td{add citation here again for the imbalance classification survey noted above to find and add (even if these are not necessarily in that survey it's fine, ie no need to check)}, 
such as Inverse of Number of Samples (INS, $w_{c}^{\text{INS}} = \frac{1}{N_c}$) and Inverse of Square Root of Number of Samples (ISNS, $ w_{c}^{\text{ISNS}} = \frac{1}{\sqrt{N_c}}$) where $w_c$ is the weight for class $c$ and $N_c$ is the number of instances in class $c$.
% \begin{equation}
%     w_{c}^{\text{INS}} = \frac{1}{N_c}
%     \label{eq:ins}
% \end{equation}
% \begin{equation}
%     w_{c}^{\text{ISNS}} = \frac{1}{\sqrt{N_c}}
%     \label{eq:isns}
% \end{equation}
To unify the above equations and allow for more flexibility in adjusting the weights, we utilize $w_{G, p}= \frac{1}{{N_G}^p}$ where $N_G$ is the number of users in the group $G$ and $p$ is for different weight assignments. INS and ISNS are two special cases with $p=1$ and $p=0.5$.
% \begin{equation}
%     w_{g, p}= \frac{1}{{N_g}^p}
%     \label{eq:power}
% \end{equation}

After updating the objective function, we train the model similarly to what we do with the baseline. Compared with the original objective function with the single goal to improve the utility performance, the updated objective function considers utility and fairness simultaneously. Here, we can balance these two goals by changing $p$. When $p=0$, it becomes the original training in baselines aiming for higher utility while increasing $p$ starts the journey towards equitable re-weighting of minority user groups. 





\subsection{Re-ranking Towards Fairness: Mitigating Group Calibration Imbalance}
% Re-ranking strategies have been utilized to improve fairness in recommender systems~\cite{}. As a post-processing method, it can be easily aggregated to existing models without re-training. It can be applied to the baseline models or to the improved models after the re-weighting strategy.

Calibration in recommendation is the property that the genre distribution (e.g., Sci-Fi, Romance, etc. in movie recommendation) in the recommendation list should match the distribution in the history interactions~\cite{steck2018calibrated}. A higher-quality calibration means a lower level of inconsistency between the distributions, which indicates that the model can better preserve users' preferences. In dating recommendation, a good calibration requires the ratios of males/females in training and recommendation to be similar. We quantify the calibration score of a user $u$ with the inconsistency between the ratio of female users that are interacted in the training dataset (i.e., $T^F(u)$) and the ratio of females that are recommended in the recommendation list $\mathcal{R}_u$ (i.e., $R^F(\mathcal{R}_u)$) by the absolute value and quantify the calibration of a group by averaging the users in that group as follows:
% preference revealed by the female ratio (the male ratio will have a similar result) between the training dataset and the recommendation. \yw{not inconsistency is calibration, but correct the inconsistency is called calibration} This inconsistency is also called calibration~\cite{steck2018calibrated} which is typically quantified by a distribution distance. Since we only have two categories (Male/Female) here rather than multiple categories (e.g., action, romance, Sci-Fi, etc for movie categories), we quantify the inconsistency of a user with the simple absolute value and quantify the inconsistency of one group with the average as follows:
\begin{equation}
    \Delta_{\text{User}}(u, \mathcal{R}_u) = |T^F(u)-R^F(\mathcal{R}_u)|, \hspace{3ex}  
    \Delta_{\text{Group}}(G, \mathcal{R}) = \sum_{u \in G} \Delta_{\text{User}}(u, \mathcal{R}_u),
\end{equation}
%\yy{necessary to include Ru since it will be changed when we adjust the recommendation in greedy algorithm}
% where $\mathcal{R}_u$ is the recommendation list for user $u$, $T^F(u)$ is the ratio of female users that user $u$ has interacted in the training dataset
% \yw{what is female ratio, I think probably rephrase this to be is the ratio of female users to the total number users that have been dated by user $u$.}
% and $R^F(\mathcal{R}_u)$ is the ratio of females in user $u$'s recommendation list $\mathcal{R}_u$. 
The group calibration result of baseline models is shown in Fig.~\ref{fig:unfairness_reasons}(b), where a low calibration score indicates better calibration. We observe that the levels of calibration differ among groups divided by OGR. It shows an opposite trend with the performance in Fig.~\ref{fig:baselines} that $G_3$ has the lowest calibration score and the highest performance. We posit that utility performance is negatively correlated with calibration scores.
% (i.e., when the calibration score is low, the performance would be high). 
Since the trained model is more towards the majority, the ability to preserve the users' preferences is compromised for the minority, leading to a poorer calibration for the minority than the majority.
% \yw{This sentence is too long and so complex, I didn't quite understand. Please rephrase in a more concise way.} 
Based on this hypothesis, we aim to mitigate the calibration imbalance issue by reducing the inconsistency between the gender ratio of training interactions and the recommendation list by re-ranking strategy. The minority has poor calibration, which on the other hand, indicates a large space for improvement. Therefore, by ensuring better calibration, it can potentially improve the utility performance of all groups with a larger improvement for the minority group, which will lead to the decrease of the utility performance gap and thus improve fairness.
% which can mitigate the performance gap and therefore improve fairness.
% reduce the inconsistency \yw{between the gender ratio of recommendation list and training interactions by re-ranking}by adjusting the gender ratio recommendation list to match more with the training interactions through re-ranking.\yw{It would be better to not use by and through together}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{Figures/inconsistency.png}
%     \caption{Inconsistency Between Training Interaction and Recommendation.}
%     \label{fig:inconsistency}
% \end{figure}

The re-ranking strategy is a post-processing mechanism, which aims to find a new recommendation list based on the original recommendations from baseline models by not only focusing on the utility performance but also on the calibration. With such consideration, we use the following objective to determine the recommendation list $\mathcal{R}_u^*$ for user $u$ based on Maximum Marginal Relevance (MMR), which is used in \cite{carbonell1998use, steck2018calibrated, zhao2021rabbit}.
% where
% we determine the reranked recommendation list 
% we leave out the subscript for brevity as the objective is the same for all users.
% The objective for selecting the recommendation list $\mathcal{R}_u$ for user $u$ is as follows, where we leave out the subscript for brevity as the objective is the same for all users.
\begin{equation}
    \mathcal{R}_u^* = \argmax_{\mathcal{R}_u, |\mathcal{R}_u|=\text{K}}(1-\lambda)S(\mathcal{R}_u)-\lambda \Delta_{\text{User}}(u, \mathcal{R}_u)
    \label{eq:mmr}
\end{equation}
% \yw{Find a better way to rephrase the description of this equation along the equation itself, I didn't quite understand this equation, why optimizing this equation could help find a better recommendation list, I didn't quite follow the logic here. Also the definition of fu(R) is not qute clear even though there is a equation here}
The objective is composed of two terms with trade-off parameter
% where $\mathcal{R}_u$ is the potential recommendation list, and $\mathcal{R}_u^*$ is the optimal recommendation list which satisfies both the utility goal and the goal to improve calibration. 
$\lambda\in [0,1]$: %controlling the tradeoff: 
(1) the predicted relevance score $\hat{y}_{ui}$ from baseline models related to the utility performance, where $S(\mathcal{R}_u)=\sum_{i\in \mathcal{R}_u}\hat{y}_{ui}$; and (2) the calibration score $\Delta_{\text{User}}(u, \mathcal{R}_u)$. Additionally, as $\Delta_{\text{User}}(u, \mathcal{R}_u) \in [0, 1]$, we rescale the relevance scores so that they fall in the same range.
% Since a better calibration entails a low calibration score, we use the negative in the maximization problem.
% \yw{I didn't quite understand why this equation could express the utility} 
Solving Eq.~\ref{eq:mmr} is an NP-hard problem~\cite{steck2018calibrated}. We adopt a greedy algorithm~\cite{nemhauser1978analysis} as in Algorithm~\ref{alg:greedy}, which finds the approximate solution with $(1-\frac{1}{e})$ optimality guarantee. To recommend potential partners for a user $u$, Algorithm~\ref{alg:greedy} starts with an empty list with top $100$ individuals recommended from the original baseline models as the candidate set $\mathcal{C}_u$ and then iteratively adds the optimal individual that obtains the largest score considering the utility and calibration under the trade-off controlled by $\lambda$. The algorithm ends when the list reaches the expected length $K$.
% \td{here do we want to say top 100, or just top K' where K'>K, probably better to be general in the algorithm and then can end with saying K'=100 or save that until the experiments when K=20 and K'=100}
% \yy{sure, can be generalized to K', updated}

\setlength{\textfloatsep}{2pt}
\SetAlgoNoEnd
\begin{algorithm}[tb]
\small
 \DontPrintSemicolon
 % \footnotesize
 \KwIn{Recommendation number $K$; user id $u$; trade-off parameter $\lambda$, $u's$ top $K^\prime$ baseline recommendations as candidates $\mathcal{C}_u$} 
% \KwIn{Recommendation number $K$; user id $u$; parameter to control the trade-off $\lambda$, top 100 recommended individuals for user $u$ from baselines as candidate $\mathcal{C}_u$}

 $\mathcal{R}_u = \{\}$

 
 \While{$|\mathcal{R}_u|\leq \text{K} $}{
   $i^* = \argmax_{i \in \mathcal{C}\setminus\mathcal{R}_u} (1-\lambda) S({\mathcal{R}_u \cup \{i\}})- \lambda \Delta_{\text{User}}(u, {\mathcal{R}_u \cup \{i\}})$

    $\mathcal{C}_u={\mathcal{C}_u \setminus \{i^*\}}$
    
   $\mathcal{R}_u = {\mathcal{R}_u \cup \{i^*\}}$
    
}
\KwRet{User $u$'s re-ranked recommendation list $\mathcal{R}_u$}

\caption{Greedy Algorithm for Re-ranking Towards Improved Calibration}
\label{alg:greedy}
\end{algorithm}


